NEEDED: Introducing Hierarchical Transformer to Eye Diseases Diagnosis

With the development of natural language processing techniques(NLP), automatic diagnosis of eye diseases using ophthalmology electronic medical records (OEMR) has become possible. It aims to evaluate the condition of both eyes of a patient respectively, and we formulate it as a particular multi-label classification task in this paper. Although there are a few related studies in other diseases, automatic diagnosis of eye diseases exhibits unique characteristics. First, descriptions of both eyes are mixed up in OEMR documents, with both free text and templated asymptomatic descriptions, resulting in sparsity and clutter of information. Second, OEMR documents contain multiple parts of descriptions and have long document lengths. Third, it is critical to provide explainability to the disease diagnosis model. To overcome those challenges, we present an effective automatic eye disease diagnosis framework, NEEDED. In this framework, a preprocessing module is integrated to improve the density and quality of information. Then, we design a hierarchical transformer structure for learning the contextualized representations of each sentence in the OEMR document. For the diagnosis part, we propose an attention-based predictor that enables traceable diagnosis by obtaining disease-specific information. Experiments on the real dataset and comparison with several baseline models show the advantage and explainability of our framework.

==> prediction_model.tex <==
As shown in the Figure \ref{fig:fra}, the disease prediction model mainly consists of MOMER Information Encoder and Disease-Specific Information Extractor. The encoder based on the Transformer is used to extract textual information from MOEMR. The extractor based on Label-wise Attention is used to obtain disease-specific information for making the diagnosis. 

Transformer and its variants have exhibited powerful capabilities in many fields, including Clinical NLP\cite{li2021neural}. We briefly describe the architecture of the Transformer model, and for more details, we recommend reading the article by Vaswani et al.\cite{vaswani2017attention}
The Transformer model is usually composed of an embedding layer and several Transformer blocks (i.e., Transformer layer) stacked on top of each other. A transformer block consists of a Multi-Head Attention Layer, Feed-forward Network Layer, Layer Normalization Layer, and Residual Connections. 

%A transformer block consists of Multi-Head Attention Layer, Feed-forward Network Layer, Layer Normalization Layer and Residual Connections. 

% Given an input token sequence $X = [x_1, x_2, \dots, x_t]$,  the transformer first input it into the embedding layer to obtain the embedding representations of each token in this sequence,which can be noted as $X^{(0)}=[x_{1}^{(0)}, x_{2}^{(0)}, \ldots, x_{t}^{(0)}]$. After that, $X^{(0)}$ is processed through N layers of Transformer layer to get the final output $X^{(N)}$. The operations performed by the Transformer at its $l_{th}$ layer can be formulated as:

% \begin{equation}
% Z=LayerNorm(X^{(l)}+ MultiHead (X^{(l)}, X^{(l)}, X^{(l)})
% \end{equation}
% \begin{equation}
% X^{(l+1)}=LayerNorm(Z+\mathcal{F}(Z))  
% \end{equation}

% Where $X^{(l)}$ is the input of $l_{th}$ layer of transformer, $\mathcal{F}(\cdot)$ denotes a feed-forward network, and $MultiHead(\cdot)$ denotes the multi-head attention operation. Multi-head attention is one of the key module of transformer, which enable the model to jointly attend to information from different representation subspaces at different positions. Multi-head attention consists of several attention layers running in parallel. Each attention head takes three inputs: $Q, K, V$; to perform the scaled dot-product attention according to Equation 2. 

% \begin{equation}
% \begin{aligned}
%  { MultiHead }(Q, K, V) &= { Concat }({ head }_{1}, \ldots,  { head }_{\mathrm{h}}) W^{O} \\
%   {where} \quad { head }_{\mathrm{i}} &= { Attention }(Q W_{i}^{Q}, K W_{i}^{K}, V W_{i}^{V})
% \end{aligned}
% \end{equation}
% \begin{equation}
% Attention(Q,K,V) = softmax(\frac{QK^T}{\sqrt{d_k}})V
% \end{equation}
% Where $W^{Q} \in \mathbb{R}^{d_{\text {model }} \times d_{k}}, W^{K} \in \mathbb{R}^{d_{\text {model }} \times d_{k}}, W^{V} \in \mathbb{R}^{d_{\text {model }} \times d_{v}}$.
% Compared with single attention operation, Multi-head Attention will to linearly project the queries, keys and values $h$ times with different, learned linear projections to $d_k, d_k$ and $d_v$ dimensions, respectively.
% On each of these projected versions of queries, keys and values will be performed the attention operation in parallel, yielding $d_v$-dimensional output values. Then,the outputs from different self-attention operations are concatenated and performed linear mapping operation.



\subsection{MOEMR Information Encoder} 

% Like some common text classification tasks, a simple way to encode an MOEMR document to obtain its embedding representation is to concatenate all sentences into a sequence of words, then use Transformer or other models to obtain an embedding representation of each word, and finally obtain the embedding representation of the MOEMR by averaging pooling or other operations on each word representation.
% However, this simple approach has obvious limitations. First, it only considers MOEMR as a sequence of words, without taking into account the differences between the types of information contained in its different kinds of texts.  
% Second, the content of MOEMR documents varies greatly in length, and processing them in this way for longer MOEMR documents can lead to excessive computational effort for the Transformers model. 
% Third, this approach first obtains representations of each word, and then obtains representations of the document directly based on these word representations, without considering that the information needed to focus on diagnosing different diseases is different. Furthermore, we can assume that this approach treats words as the minimal meaningful semantic units.
% However, we consider that the type information of the text should be preserved when encoding MOEMR documents and that sentences should be treated as the minimal meaningful semantic units rather than words.
% Therefore, we propose a Transformer-based hierarchical encoder to extract the information in MOEMR.

As shown in Figure \ref{fig:model}, the MOMER Information Encoder consists of a Sentence Encoding Layer(SEL) and a Sentence Representation Interaction Layer(SRIL).
The SEL takes the MOEMR document with $M$ paragraphs $\left \{P_1, P_2, \dots, P_M\right \} $ as input, encodes each sentence in these paragraphs, and obtains their embedding representations. In this step, we preserve the type information of the sentence by adding the type-token at the beginning.
Then, SRIL takes the set of sentence embedding representations as input, models the dependencies between sentences, and outputs the contextualized representation of each sentence. 
We designed the MOMER Information Encoder with the following considerations: 
(1) As mentioned before, we consider that the minimal meaningful semantic unit for OEMR is the sentence and should preserve the type information of the sentence, so we first obtain the embedding representation of each sentence.
(2) The meaning of each sentence will vary depending on its context, so it is essential to make its embedding representation dynamically adapt to the context.
(3) The contents of MOEMR documents vary significantly in length, and for longer MOEMR documents, processing them in this hierarchical way can reduce the Transformer model's computational cost.

\subsubsection{Sentence Encoding Layer}
The SEL follows the structure of the original Transformer Encoder and contains $N_{s}$ Transformer Encoder layers. In this stage, we use the SEL to embed each sentence in the MOEMR into $d_{\text {model }}$ dimensional representation space. To retain information about the text type to which each sentence belongs, we first add a type-token $t_0$ at the beginning of each sentence to mark its type.
Then, we use SEL to obtain the contextualized representation of each token in the input sentence. Given an input sentence $s_i$ with token sequence $[t_0^{(i)}, t_1^{(i)}, t_2^{(i)}, \dots, t_{|s_i|}^{(i)}]$. The SEL outputs $H = [h_0^{(i)}, h_1^{(i)}, h_2^{(i)}, \dots, h_{|s_i|}^{(i)}]$, where $h_j^{(i)}$ is a $d_{\text {model }}$ dimensional embedding representation corresponding to $t_j^{(i)}$. Finally, we take the average-pooling of $H$ to obtain the embedding representation $a_i$ of the input $s_i$.
Formally, for each sentence $s_i$, the representation vector $a_i$ can be obtained by:

\begin{equation}
\begin{aligned}
 a_i &= Pooling([h_0^{(i)}, h_1^{(i)}, h_2^{(i)}, \dots, h_{|s_i|}^{(i)}]])\\
     &= Pooling(SEL([t_0^{(i)}, t_1^{(i)}, t_2^{(i)}, \dots, t_{|s_i|}^{(i)}])) \\
     &= Pooling((Transformer_{m}([t_0^{(i)}, t_1^{(i)}, t_2^{(i)}, \dots, t_{|s_i|}^{(i)}]))
\end{aligned}
\end{equation}

$h_i$ and $a_i$ are both $d_{\text {model }}$ dimensional vector. After encoding all sentences, we get a matrix $A = {[a_1, a_2, \dots, a_{N}]}^T$, which shape is $d_{\text {model }} \times N$. N is equal to the sum of the number of sentences in the MOEMR.

%[经过上面的Medical Record Sentence Encoder,我们获得了眼科电子病历中各个句子的独立表示。如前文所提到的,每一个句子描述的是病人的一个症状或者是一段病史。而不同症状之间以及症状和病史之间很有可能是相关的,一个症状的出现所代表的意义可能会因为其他症状的出现,或是在不同的病史情况下而有所不同。所以,对于各个句子的表示不应该只依赖于其自身的描述,还应该考虑到其他句子所包含的信息,这就要求模型能够使得不同句子表示进行交互,建模句子表示之间的依赖关系。]
\subsubsection{Sentence Representation Interaction Layer}
In the above stage, we obtain the representation of each sentence in the MOEMR document. As mentioned earlier, each sentence describes the patient's symptoms or medical history. There is likely a correlation between different symptoms and between symptoms and medical history, which means that the meaning represented by one symptom may vary depending on the presence of other symptoms or in the context of different medical histories. Therefore, the embedding representation of each sentence should not only depend on its content but also consider its context. 
%这就要求我们的模型能够实现不同句子表征的互动,并对句子表征之间的依赖关系进行建模,以获得语境化的句子表征。%
At this stage, we use a Transformer Encoder Layer as the Sentence Representation Interaction Layer(SRIL) to model the dependencies between sentence representations to obtain contextualized sentence representations. Specifically, The SRIL takes $A$ as the input and outputs a matrix $C$ that shares the same shape as $A$, which can be formulated as:

\begin{equation}
\begin{aligned}
 C &= [c_1,c_2, \dots, c_N] \\
     &=  SRIL([a_1,a_2, \dots, a_N])\\
     &= TransformerLayer([a_1, a_2, \dots , a_N]]))   
\end{aligned}
\end{equation}


\subsection{Disease-Specific Information Extractor}
After the MOEMR Information Encoder, the MOEMR document is represented as a matrix $C \in \mathbb{R} ^{d_{\text {model }}  \times N} $, where $N$ denotes the number of sentences in the MOEMR document. A typical follow-up operation is applying a pooling operation for matrix $C$ to obtain a $d_{\text {model }}$ vector and use this vector as the input to the classifier to generate the diagnostic result. This method finally produces only one vector representation for each input and uses it for diagnosing all diseases, i.e., the information used to diagnose different diseases is the same.
%我们认为不同的疾病所关注的信息是不同的,可能有些信息对于某种疾病是重要的但对于其他疾病而言是无用的甚至是噪声。换句话说,各个句子表征对于不同疾病的重要性有所不同,就像医生在诊断不同的疾病时注意不同的症状一样。%

However, the information needed to diagnose different diseases is not identical. Some information may be necessary for diagnosing one disease but less valuable or even noise for diagnosing others. In other words, the importance of each sentence in the OEMR document varies for different diseases.
Therefore, this simple approach does not reasonable. To solve this problem, we adopt the Label-Wise Attention to obtain label-specific representation, i.e., disease-specific representation, which has been proven beneficial for multi-label classification tasks in previous studies.\cite{CAML}. 

In detail, we generally follow the practice of Mullenbach et al\cite{CAML}. In order to obtain the attention weight of each component in ${S_M}$ for disease $l$, we randomly initialize its embedding representation as $e_l \in \mathbb{R}^{d_{\text model} }$. Then, we compute the matrix-vector product ${S_M}^T e_l$ and pass the resulting vector through a SoftMax function to obtain the attention weight vector $\alpha_{l}$.
\begin{equation}
\alpha_{l}=\operatorname{SoftMax}(C^{\top}e_{l})
\end{equation}
Then,we use the attention weight vector $\alpha_{l}$ and matrix $S_M$ to compute the specific representation for disease $l$.  
\begin{equation}
v_{l} = C \alpha_{l} = \sum_{n=1}^{N} \alpha_{l, n} c_{n}
\end{equation}

\subsection{Prediction and Training}
Suppose we have a total of $d$ diseases to diagnose, after the above stage, we get a matrix $V = [v_1,v_2, \dots, v_D]$ where $=v_{l}$ is the disease-specific information representation for disease $l$.
Then, we use a set of Feedforward Neural Networks(FNNs) and the Sigmoid function to calculate the probability for each disease. 
\begin{equation}
\hat{y}_{l} = \operatorname{Sigmoid}(FNN_{l}(v_{l}))
\end{equation}

The training procedure minimizes the binary cross-entropy loss, which can be formulated as:

\begin{equation}
L_{\mathrm{BCE}}(X, y)=-\sum_{l=1}^{L} y_{l} \log (\hat{y}_{l}) + (1 - y_{l}) \log (1 - \hat{y}_{l})
\end{equation}


==> preprocessing.tex <==
\subsection{Distinction of Description} 
Like the example in Figure \ref{fig:framework}, the OMER consists of several sections, bringing together descriptions of the patient's two eyes condition from multiple perspectives.
%然而,眼科疾病诊断的目标是分别诊断双眼的健康状况。考虑到如果使用混合了双眼状况描述的原始眼科电子病历数据作为疾病预测模型的输入,可能会由于模型难以区分不同眼别的状况描述而影响单眼病情的预测效果,所以在数据预处理阶段我们首先尝试从原始眼科电子病历中分离出关于不同眼睛的文本描述,形成单眼眼科电子病历。
However, eye disease diagnosis aims to evaluate the health status of both eyes separately. Considering that if the original OEMR document with mixed descriptions of both eyes' conditions is used as the input of the disease diagnosis model, the diagnostic results of the model may be affected due to the model's difficulty in distinguishing the descriptions of different eyes.
Therefore, as shown in Figure \ref{fig:distinction}, we first differentiate the descriptions of the different eyes from the original OEMR document to form two documents, which we call Monocular Ophthalmology Electronic Medical Records (MOEMR).
It has the same structure as the OEMR, except that the content is concentrated on one eye, so its mathematical definition is identical to the OEMR.

%对于主诉和病史部分的每个句子,有些句子清楚地说明了被描述的眼睛,如 "双眼 "或 "左眼",我们能够相应地做出准确的区分。而对于那些没有明确说明被描述的眼睛的句子,两个单眼的眼科electronic medical record都保留了它们,并且我们发现这些句子一般都是比较不重要的阴性描述句子%

In this paper, we take a simple and effective approach based on the characteristics of OEMR. Specifically, each section of the OEMR can be viewed as a set of sentences. For the physical examination results section, each sentence is an examination result of a particular part of an eye, so we can easily distinguish them. For each sentence in the chief complaint and history of illness section, some sentences clearly stated the eye being described, such as "both eyes" or "left eye," so we could make accurate distinctions accordingly. For those sentences that do not clearly state the eye being described, both MOEMR documents retain them. These sentences are generally relatively unimportant asymptomatic descriptions that would be filtered out in the next step. 

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{framework.pdf}
\caption{Framework.}
\label{fig:framework}
\end{figure*}

\subsection{Asymptomatic Description Filter}
After the previous step, we obtained two MOEMRs for both eyes, and we will further process them in this step and obtain the inputs for the disease prediction module. Specifically, we find many asymptomatic descriptions in (M)OEMR  documents, such as "The eyelashes are arranged neatly without swelling and redness."
These asymptomatic descriptions contain less valuable information. Their abundance leads to a low information density of (M)OEMR documents and a high degree of similarity between (M)OEMR documents, which may lead to a decrease in the effectiveness of the diagnostic model. Therefore, as shown in Figure \ref{fig:filter}, we need to filter out the least valuable parts of the asymptomatic descriptions and thus improve the effectiveness of downstream diagnostic models. 

Since most of these asymptomatic descriptions are templated descriptions added by the doctor when writing the OEMR documents, we can filter the least valuable parts of them in a simple but effective way. We first calculate the occurrence frequency of each sentence in all MOEMR documents and later filter the sentences with a frequency higher than $B$ and are in the templated asymptomatic description corpus.

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.45\textwidth]{filter.pdf}
% \caption{Filtering of partially asymptomatic descriptions of relatively low value.}

% \label{fig:filter}
% \end{figure}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.95\textwidth]{HTL.pdf}
% \caption{The model architecture and data flow of HTL. HTL first obtains the contextualized representation of each sentence in the MOEMR document, then extracts disease-specific information representation from these sentence representations and makes a diagnosis.}
% \label{fig:model}
% \end{figure*}

==> table/overall_table.tex <==

\begin{table*}[!ht]
\renewcommand\arraystretch{1}
\centering
\caption{Performance of the different models. }\label{experiment}
\setlength{\tabcolsep}{2.0mm}{\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc|cccc}
\toprule
\multirow{2}{*}{Model}      & \multicolumn{4}{c|}{Validation Set}                                                                        & \multicolumn{4}{c}{Test Set}                                                          \\ 
           & \multicolumn{1}{c}{Macro-F1} & \multicolumn{1}{c}{Micro-F1} & \multicolumn{1}{c}{Macro-AUC} & \multicolumn{1}{c|}{Micro-AUC} & \multicolumn{1}{c}{Macro-F1} & \multicolumn{1}{c}{Micro-F1} & \multicolumn{1}{c}{Macro-AUC} & \multicolumn{1}{c}{Micro-AUC} \\ \midrule

BERT  & 81.21        & 84.28      & 92.55        & 95.61    &  80.44                     &  83.14          & 92.98     & 95.91   \\ 
CAML     & 83.71        & 81.22                        & 94.32                        & 96.09     & 82.00                        & 80.88                        & 94.41    & 96.13     \\ 
LSTM-Att & 81.55       & 80.29                       & 93.50                 & 95.68     & 80.50                       & 79.13                        & 93.82    & 95.86   \\

BERT${_\ast}$  & 87.39      & 89.73                & 95.73            & 97.33   & 87.12            & 90.33                      & 95.66      & 97.34       \\ 
CAML${_\ast}$       & 88.49   & 90.53  & 96.10   & 97.59         & 87.16       & 90.24    & 96.13  & 97.57          \\ 
LSTM-Att${_\ast}$ & 88.19                       & 91.11     & \underline{97.16}          & \underline{98.14}      & 87.09                        & 91.23                        & 96.44    & 97.64    \\\midrule
NEEDED-CONCAT    & 87.96     & 89.80      & 97.14     &   98.00        &   86.14     &  89.38         & 96.38       &  97.61         \\
NEEDED-SIM    & 87.29      & 90.58      & 96.13     &   97.51        &   85.58     &  89.89          & 96.24       &  97.65        \\
NEEDED-DS     &  88.19         & 91.31           & 96.85                  & 97.89           & \underline{87.97}     &  \underline{91.29}            & \underline{97.20}          &  \underline{97.95}              \\
NEEDED-DL     &  \underline{89.29}     & \underline{91.88}        &   96.40     & 97.67         & 87.48         & 91.00       & 96.04      & 97.44          \\ 
NEEDED$-{r}$        & 82.59                        & 82.37                        & 94.85                         & 96.46    & 81.91                        & 81.50                        & 95.27    & 96.70    \\\midrule
NEEDED        & \textbf{90.25}                        & \textbf{92.61}                        & \textbf{97.92}                         & \textbf{98.59}    & \textbf{88.07}                        & \textbf{91.61}                        & \textbf{97.94}    & \textbf{98.49}    \\\bottomrule
\end{tabular}
}}
\end{table*}
